Simplicits: Mesh-Free, Geometry-Agnostic, Elastic Simulation

The proliferation of 3D representations, from explicit meshes to implicit neural fields and more, motivates the need for simulators agnostic to representation. We present a data-, mesh-, and grid-free solution for elastic simulation for any object in any geometric representation undergoing large, nonlinear deformations. We note that every standard geometric representation can be reduced to an occupancy function queried at any point in space, and we define a simulator atop this common interface. For each object, we fit a small implicit neural network encoding spatially varying weights that act as a reduced deformation basis. These weights are trained to learn physically significant motions in the object via random perturbations. Our loss ensures we find a weight-space basis that best minimizes deformation energy by stochastically evaluating elastic energies through Monte Carlo sampling of the deformation volume. At runtime, we simulate in the reduced basis and sample the deformations back to the original domain. Our experiments demonstrate the versatility, accuracy, and speed of this approach on data including signed distance functions, point clouds, neural primitives, tomography scans, radiance fields, Gaussian splats, surface meshes, and volume meshes, as well as showing a variety of material energies, contact models, and time integration schemes.

==> method-old.tex <==

\section{Method}

Our method takes as input a rest-state object, defined in any geometric representation that supports evaluating an occupancy function $\Occupancy(x) \in \R^3 \rightarrow \R$, such that $\Occupancy(x) > 0$ inside the object and $\Occupancy(x) = 0$ outside.
After a short training procedure, we produce a set of skinning weights encoded by an implicit neural network that allow easy and efficient simulation of the object.

\subsection{Implicit Linear Blend Skinning}
Our formulation is an extension of linear blend skinning~\cite{Thalman89JoinDep}, which reduces the kinematics of a deforming object to a linear combination of transformations defined at $\NumHandle$ control \emph{skinning handles}, weighted by scalar skinning weights over the object. 
Past mesh-based approaches define these skinning weights at the vertices of a mesh; we instead propose to define them implicitly at each point in space as a function $\W(x) : \R^3 \to \R^\NumHandle$.
We will discretize this function as a small neural network $\W_\Params(x)$ with parameters $\Params$, described later in \secref{architecture}.
Once skinning weights $\W$ are established, the deformation space of the object is reduced to a transformation for each skinning handle $\T^j \in \R^{3\times 4} \; \forall j \in 1..\NumHandle$, and timestepping the simulation amounts to updating these transformations.
Typically $\T^j \in SE(3)$, although we will not need to enforce this property explicitly.
Precisely, the forward deformation map $\DeformationMap(x): \R^3 \to \R^3$ maps each location in the objects reference pose to a deformed location, and is given by
\begin{equation} \label{eq:lbs_equation}
  \DeformationMap_{\W, \T}(x) := x + \sum_{j=1}^\NumHandle \W^j (x) T^j \begin{bmatrix} x \\ 1 \end{bmatrix}.
\end{equation}

This formulation has two key properties.
First, the fully-implicit setup allows us to sidestep concerns of discretization, applying the same simulator on a wide range of geometric representations.
Second, no matter what function space we use to encode $\W(x)$, \eqref{lbs_equation} is \emph{linear} with respect to the reduced handle degrees of freedom $T^j$.
We are free to use a highly-nonlinear function space such as a neural network for $\W$, without concern for the difficulties of optimizing in this space at simulation-time, which has proven difficult in past work~\citep{sharp2023data,chenwu2023insr-pde}.

However, we still must compute a suitable set of skinning weights $\W(x)$ for any given input object.
Previous methods compute them explicitly on a mesh as a function of distance from keypoints~\cite{}\ns{TODO ref}, a biharmonic PDE~\cite{jacobson2011BoundedBW}, or a spectral decomposition~\cite{benchekroun2023fast}, but these approaches are not easily adapted across varied input representations beyond meshes. 
Instead, we will define a variational formulation to optimize for weights which best encode the physics of an object.

% TODO mention rotation equivariance somewhere?

\subsection{Implicit Elastic Energies}
Elastic deformations are governed by a material energy $\MaterialEnergy$, such as linear elastic, Neohookean, or Saint Venant–Kirchhoff.
Our approach is applicable to any such energy, though our experiments focus on linear elastic and Neohookean.
\ns{TODO: See \appref{details} for expressions for $\MaterialEnergy$}.
Generically, $\MaterialEnergy(z): \R^{3\times 3} \to R$ is a pointwise function, giving potential energy as a function of the \emph{deformation gradient} $\DeformationGradient_\DeformationMap(x) : \R^3 \to \R^{3\times 3}$, which is the Jacobian of the forward deformation map $\DeformationMap$
\begin{equation}
  \label{eq:elastic_energy_integral}
  \ElasticPotential := \int_{\R^3} \Occupancy(x) \MaterialEnergy(\DeformationGradient(\DeformationMap(x))) dx.
\end{equation}
Note that although the deformation is defined everywhere in space, $\Occupancy(x) = 0$ outside of the object, limiting the support of the integral.
To evaluate the elastic potential energy on a generic implicit representation, we can simply Monte-Carlo sample \eqref{elastic_energy_integral} in the domain containing the rest-pose object.


\subsection{Fitting Implicit Skinning Weights}
Good skinning weights accurately capture large, physically-plausible rotations and deformations of an object, even with a limited number of handles.
We seek to fit an implicit weight function $\W$ with these properties, \ie{} train the parameters $\Params$ of a neural network $W_\Params$.

\paragraph{Physical-Plausibility}
Material-aware and spatial-aware deformations have low elastic potential energy (\eqref{elastic_energy_integral}), while undesirable nonsensical deformations have very high elastic energy.
Accordingly, we seek weights which minimize the elastic energy for any random set of handle transformations
\begin{equation}
  \label{eq:objective_elastic}
  \LElastic := \mathbb{E}_{\T \sim \mathcal{S}} \left[ \int_{\R^3} \Occupancy(x) \MaterialEnergy(\DeformationGradient(\DeformationMap_{\W_\Params,\T}(x))) dx \right].
\end{equation}
The expectation is taken over transformations $\T$ from some distribution $\mathcal{S}$, in practice we randomly sample small rigid transformations $\T$ during training.

\paragraph{Orthogonality} 
Unfortunately, naively minimizing $\LElastic$ immediately collapses to a trivial solution, with all handles encoding a constant weight, limiting the model to rigid motions.
This could be mitigated in a ``supervised'' manner, by requiring the skinning weights to reproduce some dataset of motions, but such a datasets are rarely available in practice.
Instead, we adopt a data-free approach \citep{sharp2023data}, additionally seeking weights which are mutually orthonormal under the inner product on scalar functions $\int\! f(x) g(x) dx$, which amounts to minimizing
\begin{equation}
  \label{eq:objective_orthogonal}
  \LOrtho := \sum_{i=1}^\NumHandle \sum_{j=1}^\NumHandle \left(\int_{\R^3} \Occupancy(x) \W_\Params^i(x)\W_\Params^j(x) dx - \delta_{ij} \right)^2
\end{equation}
where $\delta_{ij}$ is the Kronecker delta.

\paragraph{Combined Objective}
The weight fitting objective is a weighted combination of these terms
\begin{equation}
  \label{eq:objective_combined}
  \Params^* := \text{argmin}_\Params \ \WElastic \LElastic + \WOrtho \LOrtho
\end{equation}
with spatial integrals in $\LElastic$ and $\LOrtho$ evaluated via sampling of the domain.
See \secref{something} for training details and hyperparameters.
The result is a fitted implicit weight function $\WOpt$ for the shape, which smoothly captures large nonlinear deformations.

\subsection{Time-stepping}
% Here we discreetly start being a bit more discrete
Once the skinning weights $\WOpt$ have been fit, the object can be simulated by updating the handle transformations $\T$ as degrees of freedom.
This is now a standard integration setup; the dynamics of the object are determined by the elastic energy, as well as any other terms introduced to system, such as gravity, contact, or penalty forces. Any standard integrator could be used; we find Backwards Euler to be effective. 

To evaluate the timestep, we consider a set of stochastic sample points $p$ covering the rest pose of the object. 
Recall that the deformed position of a point $p$ at time $t$ is
\begin{equation}
  p(\T_t) = \DeformationMap_{\W, \T_t}(p) = p + \sum_{j=1}^\NumHandle \W^j (p) T^j_t \begin{bmatrix} p \\ 1 \end{bmatrix}.
\end{equation}
We can then write the implicit timestep as \ns{TODO nick work in progress, stopping here...}
\begin{equation}
  \T_{t+1} = \text{argmin}_\T \int_\R^3 
    \label{eq:discreteMinimization}
\end{equation}


For a set of 
\begin{equation}
    \W^* = \text{argmin} \; \sum_{i=0}^{|\SP|} \alpha_1\MaterialEnergy(\zeta_i) + \alpha_2\|\W(\SP)^T\W(\SP) - \mathbf{I}\|^2,
    \label{eq:discreteMinimization}
\end{equation}


Although $\T$ intuitively represent rigid transformations, we find it simple and effective to optimize them as unconstrained $\R^{3 \times 4}$ matrices; the elastic energy ensures that the resulting object deformations are approximately rigid locally.


\subsection{Discretizations}
In practice, we integrate ~\autoref{eq:minimization} over $\R^3$ by using the density term $\Occupancy$ to randomly sample a set of points with positive density, $\SP \subset \R^3$. We use the same LBS equation in ~\autoref{eq:lbs_equation} to determine the deformation, $\zeta$ for any $x \in \SP$ given $\NumHandle$ handle transforms $\T \in \R^{3\times 4 \times \NumHandle}$ and a skinning weight function $\W(x) \in \R^3 \rightarrow \R^1$. We emphasize that $\SP$ are simply Monte Carlo sampled integration primitives ("cubature points") used to compute the energy over the object. We do not need to judiciously select these points, and, during optimization for $\W^*$, we randomly sample a new $\SP$ at each training iteration. 

\subsubsection{Discrete Optimization}
At the start of iteration $k$, we sample $\SP^k$ from the object. We query the material properties $\rho$ (density), $\lambda, \mu$ (lame parameters) at each cubature point which we use to compute the energy. Next, we deform $\SP^k$ by applying a set of normally sampled transforms, $\T^k \sim \NDist(\mean, \stddev)$, and evaluating \autoref{eq:lbs_equation} using $\W^k$. Unlike ~\citet{benchekroun2023fast}, we find that we can sample the entire handle transformation space, rather than just the handle translations because we have the ability to explicitly update hyperparameter $\stddev$ such that the sample deformations are proportional to the object size, thus preventing the weights from collapsing to 0 \vm{Dave is this too much explanation??}.

We compute the loss,
\begin{equation}
    \W^* = \text{argmin} \; \sum_{i=0}^{|\SP|} \alpha_1\MaterialEnergy(\zeta_i) + \alpha_2\|\W(\SP)^T\W(\SP) - \mathbf{I}\|^2,
    \label{eq:discreteMinimization}
\end{equation}
where we sum the elastic energy, $\MaterialEnergy$, with the orthogonality term, and auto-differentiate for the gradients. Regardless of the specific elastic energy term used in the optimization (we use neohookean and linear as specified in ~\autoref{section:ImplementationDetails}), to compute $\MaterialEnergy$, we need the deformation gradient at each "cubature point", $F_i = \partial \zeta_i(\W, \T, x) / \partial x_i$. We compute $F_i$ via auto-differentiation (or alternatively finite differences). The orthogonality term is straightforward to compute since $\W(\SP)$ is a matrix where each row $i$ corresponds to $\W(x_i) \forall \; i = 1..|\SP|$ in batched form. With the energy and auto-differentiated gradients, we can update the skinning weights function to $\W^{k+1}$ and restart the next step, $k+1$ . 

\subsubsection{Discrete Time-Stepping}
Armed with the optimal skinning function $\W^*$, we can proceed to randomly sample $p$ cubature points $\SP$ to simulate the object. We construct a basis matrix $B \in \R^{3p \times 12n}$ that maps LBS to a matrix-vector multiplication $\flatten(\zeta) = Bz$ where $z  = \flatten(\T) \in \R^{12n}$ are the flattened handle transforms. We also query the material parameters corresponding to $\SP$. Commonly used in elastodynamics, we use the implicit Euler integrator to find the updated DOFs, written as
\begin{equation}
    \begin{split}
        0 = \z_{i+1} -  \z_i - h\Dot{\z}_{i} - h^2 M^{-1}f(B\z_{i+1}) \\ 
    \end{split}
    \label{eq:backwardsEuler}
\end{equation}
are the flattened handle transforms, $h$ is the timestep, $M = B^TM_pB \in \R^{12n \times 12n}$ is the generalized inertia matrix created with the lumped, point-wise mass matrix $M_p$ from the object's cubature points, and $f$ integrates forces over the these points, $\flatten(\zeta) = B\z$. Solving ~\autoref{eq:backwardsEuler} is akin to zero-ing the gradient of
\begin{equation}
    \begin{split}
        \arg\min_{z_{i+1}} \z_{i+1}^T M\z_{i+1} -  \z_{i+1}^T M\z_i - h \z_{i+1}^T M\Dot{\z}_{i} + h^2 E(B,\z_{i+1}) \\ 
    \end{split}
    \label{eq:simMinimization}
\end{equation}
thus turning the time-stepper into an optimization solved using Newton's method. Note that $E(B, \z_{i+1})$ integrates energies over the object at each cubature including elastic energy, gravitational potential energy, penalty energies for Dirichlet boundary constraints, and log-barrier contact energy (see appendix for details and ~\cite{nocedal1999numerical} Ch.~19.6 for log-barrier reference).

\subsubsection{Rendering}
At each step of the simulation, we solve for a set of skinning handle transformations. Having a continuous skinning weight representation allows us a lot of flexibility. As demonstrated in ~\autoref{fig:Rendering_Link}, we can apply LBS using the $\T$ for each timestep on any set of points on the geometry, vertices of a mesh, dense sample points within the volume, in fact, even for nearby points outside the representation. We can use our method to deform and display the whole bounding box for an SDF and reconstruct the deforming object at each timestep via marching cubes. The options are endless.
\begin{figure}
     \centering
     \includegraphics[width=\columnwidth]{figs/SDF-Link.pdf}
     \caption{The deforming geometry can be displayed in many different ways. One might render the deformation of the surface mesh, or render it as a point cloud, visualize the deforming signed distance function, or finally reconstruct the updated geometry at each step using marching cubes.}
     \label{fig:Rendering_Link}
\end{figure}

\subsubsection{Rendering 3D Gaussian Splats}
We demonstrate the robustness of \ourmethod{} by showing how it applies to  \cite{kerbl3Dgaussians}, which represents shapes with a large finite number of 3D Gaussian Splats with anisotropic covariance. In this case, we cannot infinitely sample for smooth gap-free deformations. Instead, we limit sampling to the full support set of Gaussian particles. In addition, during the simulation phase, transformations are applied to the mean and covariance of each Gaussian:

\begin{equation}
    \begin{split}
        \mu'_i = \zeta_i (\W, \T, \mu_i) \\ 
        \Sigma'_i = F_i \Sigma_i F_{i}^{T}
    \end{split}
    \label{eq:gsplats}
\end{equation}

where  $\zeta_i$ is the linearly blended matrix that maps each Gaussian to the deformed space, and $F_i = \partial \zeta_i(\W, \T, x) / \partial x_i$ is the deformation gradient.
Specifically, we update the covariance component using the deformation gradient to ensure the Gaussian's anisotropic shape transforms correctly under large deformations (\autoref{fig:Gsplat_results}).
% (Figure~\cite{fig:Splat_object}).


% \vm{Unlike continuous neural fields, like NeRF or SDFs, Gaussian Splats  finite in number and cannot be directly infinitely sampled for smooth gap-free deformations. However, during simulation, we update the covariance and rotations of the splats by the deformation gradient to ensure no gaps appear even at extremely large deformations such as ~\cite{fig:Splat_object} <- fill in when Or sends figure}

\subsection{Implementation Details}\label{section:ImplementationDetails}
Our entire implementation is written in Pytorch and runs entirely on the GPU. We use an RTX 3070 for the training and simulation timings in the table. We use Blender and Polyscope to generate our results.

\subsubsection{Weight Function Approximation}
We approximate the skinning weight function using a multi-layer perceptron (MLP) for $\W$. The MLP parameters are included in the table of examples in the appendix. We use the non-linear ELU activation function, although we find that for smaller deformations, Siren activation produces similar results. 
Unlike classic skinning formulations, where the weights $\W$ are defined as a partition of unity, or at least positive, we find it effective in practice to leave $\W$ unconstrained in $\R^\NumHandle$ akin to skinning eigenmodes~\cite{benchekroun2023fast}.


\subsubsection{Training Details}
We train on batches of 10 randomly sampled sets of deformations, $\T$, at each training step. We find that for large objects using $T \sim \NDist(1, 0)$ produces very large elastic energies, and we must use $T ~\sim \NDist(\mu, 0)$ with $\mu\ll1$ to ensure that orthogonality loss can decrease sufficiently. We find that $\mu = 0.1$ works well for our large examples. Additionally, a learning rate scheduler is found to be helpful in some examples, as well as a linear scheduler for energy type. An $\NumHandle$ step training process starts off minimizing linear elasticity and ends with Neohookean elasticity $\MaterialEnergy = \frac{i}{n}\Psi_{neo} + (1 - \frac{i}{n})\Psi_{lin} \; \forall i = 0..n$. To be clear, this is during training and simulation \emph{only} uses the Neohookean term. We calculate the elastic energies as 
\begin{align}
\begin{split}
    &J = \detr(F), \;\; \; I1 = \tr(F^T F), \;\; \; \epsilon = \frac{1}{2}F^TF - I \\
    &\Psi_{neo} = \frac{1}{2}\mu (I1 - 3) - \frac{1}{2}\lambda(J-1)^2 \\
    &\Psi_{lin}= \mu \tr(\epsilon^T\epsilon) + \frac{\lambda}{2}\tr(\epsilon)^2
\end{split}
    \label{eq:elasticEnergy}
\end{align}
\subsubsection{Simulation Details}
While in principle, we could resample $\SP$ at each timestep, we find that keeping the sample set constant allows us to compute the simulation constants (like $M$ or $B$) once, up-front. As shown in the table, simple examples need fewer cubature samples, while contact examples need many more.
One drawback of the log-barrier contact penalty is "ghost forces" that remain between the two contacting objects. We find that iteratively stiffening the barrier by increasing the coefficient reduces these "ghost force" effects at the cost of a Newton solve at each update of the barrier stiffness.


In our Newton's Method, we calculate an auto-differentiated force vector of size $12n$ and an analytical stiffness matrix of size $12n \times 12n$ as outlined in the supplementary material. We solve for the Newton search direction and use a backtracking line search to find the step size. To ensure the invertibility of the hessian, we use the local hessian update from ~\citet{smith2018stable} to ensure the hessian is symmetric and positive definite.

% ==== GRAVEYARD ======

% In our linear blend skinning (LBS) formulation, the deformation of a point $x \in \R^3$ is parameterized by $\NumHandle$ handles $\T^j \in \R^{3\times 4}$, each of which encodes an arbitrary $3 \times 4$ handle transformation. Typically $\T^j \in SE(3)$, but we do not enforce this explicitly. The transformations are linearly weighted by a skinning weight function $\W(x) \in \R^\NumHandle$ resulting in the deformation 
% where $\zeta_i \in \R^3$ is the deformed point, set by a linear combination of skinning handles $\T^j \in \R^{3\times4} \forall \; j = 1..\NumHandle$, and weighted by skinning weights $\W^j(x) \in \R^1$. At rest, $\T := 0$, and $\DeformationMap = x$. 
% Previous, mesh-based formulations such as \cite{jacobson2011BoundedBW, Jacobson2012FastAS} compute skinning weights $\W$ as a function of the mesh geometry such as distance or a biharmonic relation, and store it as a discrete field at the mesh vertices. Instead, we propose to define $\W$ as a general neural function, and optimize it directly against a deformation objective. This formulation generalizes skinning weights to an extremely broad class of geometric representations, while the optimization-based formulation can automatically find high-quality weights.
%

% In order to do this, the skinning function should be material-aware, spatially-aware, and high-resolution. \citet{benchekroun2023fast} have made great progress towards such weights, but their formulation is mesh-resolution dependent, requires a linearization of the non-linear material energy, and an expensive eigenvalue solve, which scales poorly as object resolution increases \ns{do we really need to bring prior work up again here? why not leave it for related work or results?}. Our method optimizes a weight function that produces material-aware, spatially aware, and rotationally equivariant weights without requiring a linearization of the material energy or an eigenvalue solve. We swap the poor scalability of an eigenvalue solve on the stiffness matrix of a dense mesh for a resolution-independent optimization problem. Our skinning weights capture large rotations, and non-linear deformations and are \textit{continuous in space} and thus independent of object resolution. Our minimization,
% \begin{equation}
%     \W^* = \text{argmin} \; \int_{\R^3} \alpha_1\MaterialEnergy(F(\zeta, x)) + \alpha_2 \sum_{i=1}^\NumHandle \sum_{j=1}^\NumHandle \left(\W^i(x)\W^j(x) - \delta_{ij} \right)^2 dx,
%     \label{eq:minimization}
% \end{equation}
% equates to finding the optimal set of $\W^j \forall \; j=1..\NumHandle$ that minimizes elastic energy, $\MaterialEnergy$, while maintaining orthogonality between any two $\W^j, \W_m \in \W$. We sum $\MaterialEnergy$ over all of $\R^3$ since only points with non-zero density $\Occupancy$ will contribute to the elastic energy. The deformation gradient, $F = \frac{\partial \zeta}{\partial x}$, measures the deformation at all points $x \in \R^3$. We set coefficients $\alpha_1 << \alpha_2$ to ensure that our skinning handles do not all control the same sections of the object. 
%
% To fit the weights, at each optimization step $k$, we first randomly transform $\T$ and linearly blend with the current $\W$ over the geometry to deform any point $x \rightarrow \zeta$. Next, we calculate the elastic energy, $\MaterialEnergy$, and orthogonality loss for that deformation and set of fields. Finally, we get the gradients of the total loss and update $\W \rightarrow \W^{k+1}$. Eventually, this converges to a weight function with a smooth weight field for each handle $j$ which is spatially orthogonal to the weight fields for other handles, and together the fields capture large non-linear deformations in the object. Essentially, our skinning weight function produces continuous weight fields that act as a low-energy bases of the object that is deformed by skinning handles $\T \in \R^{3\times 4 \times \NumHandle}$ \ns{this sentence seems redundant with previous text}.\vm{it is. I find these rephrased/tldrs helpful when I'm reading papers.}
%


==> related_work_new.tex <==
\section{Related Work}

Mesh-based elasticity simulation has long been a part of computer graphics~\citep{Terzopoulos1987}. The most common variant in use today, for volumetric simulation, is the linear tetrahedral finite element method~\citep{cutler2002procedural}. Since its initial introduction to graphics there have been fundamental improvements in performance~\citep{bargteil2007finite,bouaziz2014projective,macklin2016xpbd}, extensions to more complicated phenomena~\citep{bargteil2007finite} including contact~\citep{liincremental} and higher-order implementations~\citep{Schneider:2019:PFM,Schneider:2018:DSA}. In our context the most important advancements have been made in the geometry processing pipeline which constructs volumetric tetrahedral meshes from surface input where robust tools~\citep{Hu2018,diazzi2023constrained} enable virtually black box of such geometry. 

However, even broadening the scope of input geometry slightly increases the complexity of the geometry processing and simulation pipelines significantly. For instance objects with thin features either force volumetric mesh resolutions be exceedingly high (impractical for many applications) or require special co-dimensional treatments which allow for the inclusion of medial axis geometry (lines for rods and sheets for triangles) into the simulation. Specialized simulators exist for geometry solely constructed from thin primitives~\citep{baraff2023large,bergou2008discrete} but, coupling these to volumetric approaches requires non-trivial solutions~\citet{chang2019unified,Li2021CIPC})

In such cases, an attractive alternative are embedded methods, which wrap any and all geometry inside an easily constructable discretization~\citep{longva2020higher}. These can produce excellent results but will naively couple disparate geometric elements embedded in the same element, again necessitating additional algorithmic modifications~\citep{nesme2009preserving}.

Alternatively, one could turn to mesh-free method to simulate complex geometries. ~\citep{pauly2005meshless} since they reduce the surface geometry to volumetric conversion to effectively point sampling input geometry. For instance, \citet{peer2018implicit} can simulate objects with smooth particle hydrodynamics (SPH) given a sufficiently high particle density to build shape-aware kernels, but cannot generalize to arbitrary materials. Further the spherical nature of the kernels means they are not shape-aware. A problem that is recurrent in more recent approaches designed for simulating NeRFS~\citep{feng2023pienerf}. \citet{hu2019taichi, wolper2019cdmpm} use the material point method (MPM) to model plasticity and fracture, however, it requires an explicit which prevents it from being accurate, quantitatively or qualitatively for large-scale elasodynamics. Concurrent work for  direct simulation of Gaussian Splats inherits this limitation~\citep{xie2023physgaussian}. ~\citet{faure2011sparse} is a mesh-free simulator which uses a frame-based approach, along with precomputed weight functions to represent object kinematics. This approach is this closest to ours technically and philosophically however it still requires an explicit boundary for boundary conditions which means it cannot directly take, as input, representations such as Gaussian Splats, while our proposed approach can. Further the method requires a dense voxelization of the object for computing and storing weight-functions which is memory intensive. 

Our work is most superficially related to frame-based and skinning-based dynamics simulation~\citep{benchekroun2023fast,trusty2023subspace}. In particular we take, as a starting point, the skinning eigenweights from~\citep{benchekroun2023fast} and extend them in three major ways. First we extend the eigenweight optimization into the nonlinear regime. Second, in this nonlinear regime we show that it is possible and preferable to optimize the weights under the assumption of full affine transformations, rather than just the translations of prior work. Finally, rather than store skinning weights on a volumetric tetrahedral mesh, we store the weights as neural fields enabling a fully meshless pipeline from beginning to end. 

Leveraging neural networks and and neural fields for physics simulation is a fast growing reasearch area. ~\citet{chenwu2023insr-pde} develop a neural simulation technique that can handle infinitely high geometric resolution at a very high simulation cost per timestep (often on the order of hours). Other neural techniques pioneered by ~\citet{Fulton2019} can alleviate some of the issues related to simulation speed via reductions to a nonlinear, neural latent space. Recently, this idea was further refined as Continous-Reduced Order Models (CROM) ~\citet{chen2023crom,chang2023licrom} which use prior simulation data to generate reduced order models for simulation. However these methods rely on explicit meshes, explicit mesh gradients and the availability of pre-simulated datasets -- thus inheriting the geometry processing challenges described above, but in the training rather than runtime portions of the method. This again limits their applicability to a large range of geometric applications without further algorithmic development. In contrast, our data-free training is inspired by the neural method developed by ~\citet{sharp2023data} which optimizes a neural network to learn the low-order subspace of an explicit mesh for \textit{kinematics}. Unfortunately this method only succeeded in generating kinematic subspaces, rather than enabling dynamic simulation.

\begin{figure}
     \centering
     \includegraphics[width=\columnwidth]{figs/Explaning-SkinningModes.pdf}
     \caption{A simulation basis created through our optimization displayed via colored point samples on the object. The first basis vector is a constant over the object which enables rigid transformations.}
     \label{fig:SkinningModes}
\end{figure}

In contrast, we our nonlinear skinning optimization to learn skinning weight functions over complex domains whether they are represented by an explicit mesh or not~(\autoref{fig:SkinningModes}). \ns{need to cite ML community simulation, like deformable nerf sim stuff}. 

Our core technical contribution is our end-to-end pipeline which takes as input any geometric representation that can provide an inside-outside function for a piece of geometry and reliably produces a set of skinning weights which can be used for dynamic simulation. We show that the pipeline provides results that qualitatively match ground truth finite element simulation and exceed the accuracy of prior meshless methods (MPM, SPH). We demonstrate the generality and robustness of our method by performing over 80 elastodynamic simulations on geometry representations varying from explicit triangle meshes, to Computed Tomography volume data to Gaussian Splats -- all with a single pipeline, requiring no user modifications in either structure or parameter values. 




